ECP SOLLVE: Validation and Verification Testsuite Status Update and Compiler Insight for OpenMP

The OpenMP language continues to evolve with every new specification release, as does the need to validate and verify the new features that have been introduced. With the release of OpenMP 5.0 and OpenMP 5.1, plenty of new target offload and host-based features have been introduced to the programming model. While OpenMP continues to grow in maturity, there is an observable growth in the number of compiler and hardware vendors that support OpenMP. In this manuscript, we focus on evaluating the conformity and implementation progress of various compiler vendors such as Cray, IBM, GNU, Clang/LLVM, NVIDIA, Intel and AMD. We specifically address the 4.5, 5.0, and 5.1 versions of the specification.

==> plots.tex <==
\begin{figure*}
  \includegraphics[width=\textwidth,height=9cm]{images/OMP_4.5_summit.jpg}
  \caption{OpenMP version 4.5 on Summit}
  \subcaption[]{This plot shows the tests written in C,C++,Fortran for OpenMP version 4.5 run on Summit using various compilers (GCC,LLVM,NVHPC).These test have been run on three different versions of the compilers listed above GCC(v9.3.0,v10.2.0,v11.1.0) LLVM(v13,v14,v15) and NVHPC(v21.7,v21.9,v21.11) Later versions weren’t tested due to unavailability. A total of 228 tests were conducted of which 100 are on Fortran, 114 are on C and 14 are on C++ Taking GCC v11.1.0 into account 99.1\% of tests pass have passed. The only test that have failed on this compiler are 2 C tests out of the 114 C tests. The greatest improvement is seen across GCC with a pass rate of 89.9\% on v9.3.0 improving to 99.1\% on v11.1.0. LLVM’s performance was stagnant with a pass rate of 56.1\% because of all the Fortran tests failing.}
\end{figure*}

\begin{figure*}
  \includegraphics[width=\textwidth,height=9cm]{images/OMP_5.0_summit.jpg}
  \caption{OpenMP version 5.0 on Summit}
  \subcaption{This plot shows the tests written in C,C++,Fortran for OpenMP version 5.0 run on Summit using various compilers (GCC,LLVM,NVHPC).These test have been run on three different versions of the compilers listed above GCC(v9.3.0,v10.2.0,v11.1.0) LLVM(v13,v14,v15) and NVHPC(v21.7,v21.9,v21.11). Later versions weren’t tested due to unavailability. A total of 211 tests were conducted of which 47 are on Fortran, 151 are on C and 13 are on C++.Taking NVHPC v21.9 into account 36.5\% of tests pass have passed.The major contributing factor to the low percentage are the 109 C tests that have failed out of the 151 C tests. The greatest improvement is seen across GCC with a pass rate of 53.5\% on v9.3.0 improving to 82.4\% on v11.1.0.}  
\end{figure*}

\begin{figure*}
  \includegraphics[width=\textwidth,height=9cm]{images/OMP_5.1_summit.jpg}
  \caption{OpenMP version 5.1 on Summit}
  \subcaption{This plot shows the tests written in C and C++ for OpenMP version 5.1 run on Summit using various compilers (GCC,LLVM,NVHPC). These test have been run on three different versions of the compilers listed above GCC(v9.3.0,v10.2.0,v11.1.0) LLVM(v13,v14,v15) and NVHPC(v21.7,v21.9,v21.11) Later versions weren’t tested due to unavailability. Varied number of tests were conducted with the number of C test varying between 13-20 and a single C++ test. Taking LLVM v14 into account 46.6\% of tests pass have passed. Half of the 14 C test have failed. The greatest improvement is seen across GCC with a pass rate of 7.1\% on v9.3.0 improving to 73.3\% on v11.1.0. NVHPC’s performance was stagnant with a pass rate of 6.6\% because of all the C tests failing.}
\end{figure*}
